The Case for Claim Difficulty Assessment in Automatic Fact Checking

Fact-checking is the process of evaluating the veracity of claims (i.e., purported facts). In this opinion piece, we raise an issue that has received little attention in prior work -- that some claims are far more difficult to fact-check than others. We discuss the implications this has for both practical fact-checking and research on automated fact-checking, including task formulation and dataset design. We report a manual analysis undertaken to explore factors underlying varying claim difficulty and identify several distinct types of difficulty. We motivate this new claim difficulty prediction task as beneficial to both automated fact-checking and practical fact-checking organizations.

==> unused-material.tex <==
%\footnote{While performance on the leading synthetic dataset FEVER~\cite{fever} is higher at 76\% accuracy, the data is criticized to be biased~\cite{fever-rebuttal}. We focus on fact checking in practice which is better aligned with natural fact checking data.}
%
%For example, recent state-of-the-art performances on key natural and synthetic fake news datasets are only 44.3 \% \cite{Atanasova2020GeneratingFC} and 75.9\%\footnote{\url{https://competitions.codalab.org/competitions/18814#results}} respectively. What makes fact checking so difficult, and how might we gain additional traction on this problem? \prakhar{TODO for Jessy: the results on liar-plus are macro f1 while accuracy on fever, do we highlight this}

%We find that the challenges are multi-faceted: claim ambiguity, the gathering of evidence and the difference between humans and machines during this process, as well as inference over the evidence sources. These aspects lay at the basis of data collection processes needed for fact checking. Consequently, we highlight the importance of considering \textbf{claim difficulty} -- how hard it is to fact-check a given claim -- explicitly during corpora development. 
%Furthermore, we discuss the value of claim difficulty prediction as a component in fact checking systems (Section~\ref{}). 



==> unused/unused.tex <==

%Dataset design for ``claim + evidence'' based formulations of fact-checking have three key steps: claim sourcing, evidence sourcing and annotation sourcing. We discuss each separately.

%Claim sourcing is typically done by randomly sampling social media \cite{Mitra2015CREDBANKAL, checkthat2020}, scraping fact-checking websites \cite{Popat2016CredibilityAO, Baly2018IntegratingSD, multifc} or crowd sourcing \cite{PrezRosas2017AutomaticDO, fever}. 

%Evidence sourcing is typically done by borrowing expert sources \cite{Vlachos2014FactCT, liarplus, Atanasova2020GeneratingFC}, using search engines \cite{Popat2016CredibilityAO, Baly2018IntegratingSD, fakenewsnet, multifc} or using text corpora \cite{fever}. 

%Annotation sourcing is typically done using crowd sourcing \cite{PrezRosas2017AutomaticDO, fever, Mitra2015CREDBANKAL} or using annotations from fact-checking websites \cite{liar, liarplus, Popat2016CredibilityAO, Baly2018IntegratingSD, multifc, Atanasova2020GeneratingFC}.

%We propose the following changes and discuss them in more detail in Section~\ref{sec:claim-difficulty-analysis}. Firstly, 

%or crowd sourcing \cite{PrezRosas2017AutomaticDO, fever}. 
%We do not recommend randomly sampling claims, or taking all claims as-is. 
%these approaches will involve uncheckable claims due to the various reasons we discussed in Section~\ref{sec:claim-difficulty-analysis}, including language ambiguity and lack of sources. While one would expect machine learning models to tolerate some noise, we still need to understand to what extent uncheckable claims is present in the data, and to construct a fair test set that leads to valid conclusions.
%Yet random sampling uncheckable due to ambiguity (Section~\ref{sec:ambiguity}), or 
%Our findings on claim ambiguity
%Consider again claim 6 from Table~\ref{tab:taxonomy-examples}. The claim is hard to fact-check and is potentially not fact-checkable using web sources. As a result, all fact-checking models are likely to fail on this test set leading to modellers erroneously conclude that model performances are low. Instead, claims should be sampled in a stratified manner discarding at the very least ambiguous and not fact-checkable claims.



%or using text corpora \cite{fever}. 
%Since expert sources are unlikely to be available in practice, 
%using them would not account for the gap we have observed between expert sources and IR results. 
%A practical IR system will not be perfect and 
%may not always yield sources necessary to fact-check a claim unlike expert sources. %Moreover, even if a claim is fact-checkable from retrieved IR sources, the NLI task may be harder. 
%approaches that uses search engines \cite{Popat2016CredibilityAO, Baly2018IntegratingSD, fakenewsnet, multifc} is more realistic. 


%We see the need for claim difficulty prediction as a task, which we argue can be beneficial in multiple fronts.
%Adding claim difficulty prediction to the fact-checking pipeline can help alleviate this problem. 
%Firstly, many social media websites and news companies employ human fact-checkers, but they can easily be overwhelmed by the vast amount of content being generated today. The output from the claim difficulty prediction task can help triage and prioritize more difficult claims to be checked by human fact-checkers. 
%while easier claims are checked by fact-checking models. 
%Secondly, 
%Lastly, multi task learning (MTL) \cite{Li2019AnEE} has shown promising results for NLP and jointly solving the claim hardness prediction task with the main fact-checking task can help boost performance on the latter.



